(De-)Composing Causality in Labeled Transition Systems

In this paper we introduce a notion of counterfactual causality in the Halpern and Pearl sense that is compositional with respect to the interleaving of transition systems. The formal framework for reasoning on what caused the violation of a safety property is established in the context of labeled transition systems and Hennessy Milner logic. The compositionality results are devised for non-communicating systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{10}
\providecommand{\publicationstatus}{G. G\"ossler and O. Sokolsky (Eds.): 1st Workshop on Causal Reasoning for \\ Embedded and safety-critical Systems Technologies (CREST'16)\\
EPTCS 224, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.224.3}{10.4204/EPTCS.224.3}}
\pdfoutput=1

